Query-specific Variable Depth Pooling via Query Performance Prediction towards Reducing Relevance Assessment Effort

Due to the massive size of test collections, a standard practice in IR evaluation is to construct a 'pool' of candidate relevant documents comprised of the top-k documents retrieved by a wide range of different retrieval systems - a process called depth-k pooling. A standard practice is to set the depth (k) to a constant value for each query constituting the benchmark set. However, in this paper we argue that the annotation effort can be substantially reduced if the depth of the pool is made a variable quantity for each query, the rationale being that the number of documents relevant to the information need can widely vary across queries. Our hypothesis is that a lower depth for the former class of queries and a higher depth for the latter can potentially reduce the annotation effort without a significant change in retrieval effectiveness evaluation. We make use of standard query performance prediction (QPP) techniques to estimate the number of potentially relevant documents for each query, which is then used to determine the depth of the pool. Our experiments conducted on standard test collections demonstrate that this proposed method of employing query-specific variable depths is able to adequately reflect the relative effectiveness of IR systems with a substantially smaller annotation effort.

==> src/sup-qpp.tex <==
\para{Supervised QPP approaches}

Recent research has shown that supervised approaches, such as \cite{hamed_neuralqpp,qpp-bert,datta_deepqpp22,group_bert_qpp22}, outperform their unsupervised counterparts. The increase in effectiveness, however, comes at the cost of annotation effort involved in preparing training data, comprising ground-truth relevance assessments, to train these supervised models. The NeuralQPP method \cite{hamed_neuralqpp} involves training a pairwise model that predicts which of the queries leads to better retrieval results. The features used in \cite{hamed_neuralqpp} to train the pairwise model comprises RSVs, the term-document matrix of the top-$k$ retrieved set, and word embedded vectors as inputs. Datta et al. \cite{datta_deepqpp22} used a convolution-based deep learning approach which operates over interaction matrices of queries and top-retrieved documents instead of hand-coded features.  
More recently, \cite{qpp-bert} showed that a cross-encoder based pointwise approach, named BERT-QPP, making use of the interaction of the BERT vectors between query and document terms performs well. Instead of predicting a relative measure of query difficulty across a pair, the training objective in this case seeks to directly predict a retrieval effectiveness measure (e.g. MRR@10). Different from BERT-QPP, the authors of \cite{DBLP:conf/sigir/DattaMGG22} proposed qppBERT-PL, which first segments the top-$k$ retrieved documents into uniform-sized chunks, and applies sequence modeling over these chunks for QPP. Since qppBERT-PL was shown to outperform BERT-QPP, we employ this method in our experiments as a representative from the supervised class of QPP models.

The qppBERT-PL method thus is a function comprised of additionally of a set of \emph{learnable parameters} (different from the functions depicted in Equations \ref{eq:generic} and \ref{eq:nqc}), the values of which are optimized using a set of relevance assessments. Formally,
\begin{equation}
\phi_{\mathrm{\qppbert}} \defas f(Q, M^{(k)}, R(Q); \theta),
\end{equation}
where $R(Q)$ is a set of known relevant documents for Q and $\theta$ is the set of learnable parameters determining the neural network function $f$. 


==> tabdefs/mainres.tex <==
\begin{table}[t]
\centering
\small
\begin{adjustbox}{width=.99\columnwidth}
\begin{tabular}{@{}l@{}lll r cc cc@{}}
\toprule
& & & & & \multicolumn{4}{c}{Evaluation Metrics} \\
\cmidrule{6-9}
Set & Type & Pool & QPP & Depth & P-$r$ & K-$\tau$ & Recall & $\overline{|\mathcal{P}|}$ \\
\midrule
% DL 19
\multirow{8}{*}{\begin{turn}{90}TREC DL'19\end{turn}} & \multirow{2}{*}{BL} & CDP-Min & - & 1	& 0.9022	& 0.6336	& 0.2229 & \textbf{\underline{8.65}} \\
& & CDP-Avg & - & 3	& 0.9559	&0.7147	&0.4703 & 20.46 \\
\cmidrule{2-9}
& \multirow{4}{*}{Ours}& VDP-L & \multirow{2}{*}{NQC} & 3.37 & \textbf{0.9686} & \textbf{0.8559} & \textbf{0.5398} & 24.76 \\
& &VDP-IL & & 1.67 & 0.9241 & 0.7297&	0.2814 & \textbf{10.83} \\
& &VDP-L &\multirow{2}{*}{\qppbert} & 2.23 & 0.9228&	0.6396&	0.3864 & 16.02 \\
& &VDP-IL & & 3.06 & 0.9603&	0.7688&	0.4203 & 19.44 \\
\cmidrule{2-9}
& AL & CDP-Max & - & 5	& \cellcolor{green!25}0.9850	&\cellcolor{green!25}0.9399	&\cellcolor{green!25}0.6542 & \cellcolor{green!25} 30.67 \\
%
%DL 20
\midrule
\midrule
\multirow{8}{*}{\begin{turn}{90}TREC DL'20\end{turn}} & \multirow{2}{*}{BL} & CDP-Min & - & 1	& 0.9760	& 0.8656	& 0.2448 & \textbf{\underline{12.27}} \\
& & CDP-Avg & - & 3	& 0.9944&	0.9299 & 0.4878 & 29.48 \\
\cmidrule{2-9}
& \multirow{4}{*}{Ours}& VDP-L & \multirow{2}{*}{NQC} & 3.87 & \textbf{0.9960} & \textbf{0.9334} & \textbf{0.5740} & 37.50 \\
& &VDP-IL & & 1.67 & 0.9866 & 0.9030&	0.3161 & \textbf{15.75} \\
& &VDP-L &\multirow{2}{*}{\qppbert} & 2.44 & 0.9880	& 0.9065& 0.4297 & 25.20 \\
& &VDP-IL & & 2.79 & 0.9907	& 0.9018 &	0.4260 & 26.62 \\
\cmidrule{2-9}
& AL & CDP-Max & - & 5	& \cellcolor{green!25}0.9977	&\cellcolor{green!25}0.9568	&\cellcolor{green!25}0.6671 & \cellcolor{green!25}45.24 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\small
A comparison of QPP-based variable depth pooling with constant depth pooling approaches (including the oracle cases shown in green).}
\label{tab:mainres}
\end{table}

